Edge dynamics of an Integer Quantum Hall system

In this master thesis work the linear and non linear edge dynamics of a non-interacting system of fermions in a Integer Quantum Hall state is theoretically and numerically studied.

==> Chapters/ChapterTemplate.tex <==
%!TEX root = ../main.tex
% Chapter Template

\graphicspath{{./Pictures/X/}}

\chapter{Chapter Title Here} % Main chapter title

\label{ChapterX} % Change X to a consecutive number; for referencing this chapter elsewhere, use \ref{ChapterX}

\lhead{Chapter X. \emph{Chapter Title Here}} % Change X to a consecutive number; this is for the header on each page - perhaps a shortened title

\section{Main Section 1}
